Probabilistic Uncertainty Quantification of Prediction Models with Application to Visual Localization

The uncertainty quantification of prediction models (e.g., neural networks) is crucial for their adoption in many robotics applications. This is arguably as important as making accurate predictions, especially for safety-critical applications such as self-driving cars. This paper proposes our approach to uncertainty quantification in the context of visual localization for autonomous driving, where we predict locations from images. Our proposed framework estimates probabilistic uncertainty by creating a sensor error model that maps an internal output of the prediction model to the uncertainty. The sensor error model is created using multiple image databases of visual localization, each with ground-truth location. We demonstrate the accuracy of our uncertainty prediction framework using the Ithaca365 dataset, which includes variations in lighting, weather (sunny, snowy, night), and alignment errors between databases. We analyze both the predicted uncertainty and its incorporation into a Kalman-based localization filter. Our results show that prediction error variations increase with poor weather and lighting condition, leading to greater uncertainty and outliers, which can be predicted by our proposed uncertainty model. Additionally, our probabilistic error model enables the filter to remove ad hoc sensor gating, as the uncertainty automatically adjusts the model to the input data

==> archive/dump.tex <==
Our results perform significantly better than the constant-covariance baseline. Note that our method has a good N-sigma covariance credibility value and rejects much less measurements in the sensor gating, which means our method outputs a good uncertainty. When focusing on the localization performance without sensor gating, baseline localization results are close to measurement error. However, adding a proper covariance can boost the localization results a lot. While with sensor gating, since the constant covariance usually does not match with the measurement error, a lot of measurements are rejected. But with a proper covariance, sensor gating rejects bad measurements and thus improves the accuracy of localization especially in some challenging condition such as night. 

%***
Under sunny and snow conditions, our method achieves a good performance with uncertainty errors of 0.060 and 0.026, and localization error of 0.871 meter and 1.424 meter. As expected, night condition is much harder. The uncertainty error is 0.109 and the localization error is 8.680 meter. The uncertainty error is also visualized in \autoref{fig:eval_measurement}. These results give confidence that our approach can work well in various conditions.

==> sections/GMM.tex <==
\section{Uncertainty Quantification with Gaussian Mixture Models}\label{sec:GMM}
In a manner similar to \autoref{sec:method}, we establish a sensor error model for each database/traversal. In the case of database $l$, we employ the image retrieval pipeline using traversal $X^l$ as the query and another traversal $X^{m\neq l}$ as the database. For every image $k_i^l \in X^l$, we locate the closest image $f(k_i^l; X^m)$ from database $m$, enabling us to calculate the location error $\lVert r(f(k_i^l; X^m)) - r(k_i^l) \rVert$, where $r(f(k_i^l; X^m))$ and $r(k_i^l)$ stands for the location of image $f(k_i^l; X^m)$ and $k_i^l$. This process allows us to determine both the number of keypoint matches to its closest image and the corresponding location error for each image. We repeat this procedure for all $L-1$ different traversals, excluding $X_l$.
To analyze the data, we divide it into bins based on the number of keypoint matches. Within each bin, we fit a Gaussian Mixture Model (GMM) of 3 components on the data to effectively represent the distribution. We iterate this process for each traversal/database combination.

\subsection{Visual Localization Pipeline with Gaussian Sum Filter}
To seamlessly integrate the Gaussian Mixture Sensor Error Model into the visual localization pipeline, we employ the Gaussian Sum Filter (GSF). By incorporating the GSF, we ensure that the localization process effectively incorporates the nuanced characteristics captured by the Gaussian Mixture Models (GMMs).

% \begin{figure}[htbp]
% \vskip-5pt
%         \centering
%         \includegraphics[width=0.95\linewidth]{figures/chapter5/GAU_SUM.png}
%         \caption{\small Gaussian Sum Filter
%         \label{fig:gau_sum}}
%         \vskip-5pt
% \end{figure}

The GSF represents the probability density function (PDF) of the system state as a sum of $N_{g_{k}}$ Gaussian components, as shown by the following equation:
\begin{equation}
p(x_{k}|z_{1:k})\approx \sum_{i=1}^{N_{g_{k}}}\omega^{i}_{k}\cdot \mathcal{N}(x^{i}_{k}, P^{i}_{k})
\end{equation}
In the given equation, the variable $k$ denotes the time index and $z$ denotes the measurement. The $\omega$ represents the weight, $\hat{x}$ represents the mean, and $P$ represents the covariance of each Gaussian component. Each Gaussian component corresponds to a potential hypothesis regarding the true state of the system. By performing recursive updates, these components are progressively combined and refined over time, resulting in an increasingly accurate estimation of the state.

The Gaussian Sum Filter (GSF) operates in two main stages at each time step: prediction and update. In the prediction stage, the GSF predicts the new state estimate based on the system dynamics model. Each Gaussian component is propagated according to the model, accounting for any uncertainty or noise in the system. The prediction equation is given by:
\begin{equation}
p(x_{k+1}|z_{1:k})\approx \sum_{i=1}^{N_{g_{k}}\cdot N_{\omega}}\Bar{\omega}^{i}_{k+1}\cdot \mathcal{N}(x^{i}_{k+1}, P^{i}_{k+1})
\end{equation}

In the update stage, the GSF incorporates measurement information to refine the state estimate. In our case, the measurement is represented by a Gaussian Mixture, which is given by:
\begin{equation}
z_{k+1}= \sum_{i=1}^{N_{\upsilon}}\gamma^{i}\cdot \mathcal{N}(\mu^{i}, \Sigma^{i})
\end{equation}
where $\gamma$ is the weight, $\mu$ is the mean and $\Sigma$ is the covariance of each measurement component. The predicted Gaussian components are weighted based on a combination of their previous weights, measurement weights, and their likelihood given the measurement. These weights reflect the confidence or belief in each hypothesis. The updated state estimate equation is:
\begin{equation}
p(x_{k+1}|z_{1:k+1})\approx \sum_{i=1}^{N_{g_{k}}\cdot N_{\omega}\cdot N_{\upsilon}}\Tilde{\omega}^{i}_{k+1}\cdot \mathcal{N}(x^{i}_{k+1}, P^{i}_{k+1})
\end{equation}
\begin{equation}
\Tilde{\omega}^{i}_{k+1}=\Bar{\omega}^{j}_{k+1}\gamma^{l}p(\hat{z}^{l}_{k+1}|x_{k+1}^{j}) 
\end{equation}
where $\Bar{\omega}^{j}_{k+1}$ stands for each component weight in $p(x_{k+1}|z_{1:k})$ and $\gamma^{l}$ stands for each component weight in $z_{k+1}$.  

After the update stage, the GSF performs a pruning and merging step to maintain a tractable number of Gaussian components while still representing the underlying PDF accurately. Following Runnalls’s\cite{4383588} condensation algorithm, given two weighted
Gaussian densities $\omega^{i}\cdot \mathcal{N}(x^{i}, P^{i})$ and $\omega^{j}\cdot \mathcal{N}(x^{j}, P^{j})$ from a Gaussian mixture, the merged weight $\omega^{ij}$, mean $x^{ij}$ and covariance $P^{ij}$ are:
\begin{align}
\omega^{ij}&=\omega^{i}+\omega^{j} \\
x^{ij} &= \frac{\omega^{i}}{\omega^{ij}}x^{i}+\frac{\omega^{j}}{\omega^{ij}}x^{j}\\
P^{ij}&=\frac{\omega^{i}}{\omega^{ij}}P^{i}+\frac{\omega^{j}}{\omega^{ij}}P^{j}+\frac{\omega^{i}\omega^{j}}{(\omega^{ij})^2}(x^{i}-x^{j})(x^{i}-x^{j})^{T}
\end{align}
The condensation approach in the Gaussian Sum Filter (GSF) iteratively merges components based on a bounded approximation of the Kullback-Leibler divergence between the original and reduced mixture. This divergence $B^{ij}$ is bounded by the expression:
\begin{equation}
B^{ij}=0.5\cdot\left[(w^{i}+w^{j})\log\det(P^{ij})-w^{i}\log\det(P^{i})-w^{j}\log\det(P^{j})\right]
\end{equation}
In the GSF, pruning is applied to remove Gaussian components with low weights, indicating their reduced relevance or unlikelihood given the measurements. On the other hand, merging combines Gaussian components that are close together, reducing the number of components without significant loss of information. Through the iterative process of prediction, update, pruning, and merging, the GSF dynamically adapts to the evolving characteristics of the system and measurements. This adaptation allows it to provide an estimate of the system state that incorporates both the dynamics model and the information from the measurements.


\subsection{Experiments}

\subsubsection{Settings}
We leverage the Ithaca365 dataset~\cite{Diaz-Ruiz_2022_CVPR}, which encompasses data collected during multiple traversals along a 15km route encompassing diverse environmental conditions, including snow, rain, sunlight, and nighttime. Our experimental setup incorporates two types of sensor data: images and GPS locations. 

We conduct a comprehensive benchmark of our method against four baseline approaches: the constant covariance baseline, constant Gaussian Mixture baseline, MC Dropout, and our SPF results presented in Chapter 4. The constant covariance baseline is obtained by tuning on the validation data, separately for each weather condition.  Similarly, the constant Gaussian Mixture baseline is obtained by fitting a Gaussian Mixture Model on the validation data, individually for each weather condition. In the first experiment, we also compare our method to the Monte Carlo (MC) Dropout technique. To perform this comparison, we introduce a dropout layer after the final keypoint feature projection layer with a dropout probability of 0.3. We repeat the dropout process multiple times until the localization results using Gaussian Sum Filter stabilize, and then report the converged results. In addition, we investigate two specific study cases to simulate sensor failures: one where the measurements are corrupted by average blurring, and another where salt and pepper noise is introduced. For more information and detailed explanations, please refer to Section \ref{sec:experiments}.  

\subsubsection{Results}
% \setlength{\tabcolsep}{6pt}
\begin{table}[!bt]
\centering
\caption{Evaluation results of Gaussian Sum Filter localization with normal measurements.}
\label{table:eval_GSM}
\begin{tabular}{cl@{\hskip 0.15in}c@{\hskip 0.5in}c@{\hskip 0.45in}c}
\toprule
Row & Method & Sunny & Night & Snowy \\ 
\midrule 
\multicolumn{5}{c}{Average measurement error: 0.83m/11.67m/1.76m for MC dropout.} \\
\multicolumn{5}{c}{Average measurement error: 0.87m/8.68m/1.42m for others} \\

\midrule
1 & Constant Noise & 0.76 & 8.42 & 1.30 \\
2 & Constant Gaussian Mixture & 1.06 & 1.13 & 1.21 \\ 
3 & MC Dropout & 0.79 & 7.44 &  1.50 \\
4 & SPF & 0.56 & 3.07 & \textbf{0.81} \\ \midrule
5 & GSF & \textbf{0.57} & \textbf{1.09} &  0.84 \\
\bottomrule
\end{tabular}
\end{table}

We present the results in Table \ref{table:eval_GSM}, Table \ref{table:eval_GSM_avgblurring} and Table \ref{table:eval_GSM_snp0.5}. An analysis of the obtained results reveals several noteworthy observations. Firstly, our proposed method employing Gaussian Mixture Model and Gaussian Sum Filter consistently outperforms the baseline approaches across the majority of cases. This significant improvement indicates its superior ability to accurately quantify uncertainty. Furthermore, our method demonstrates particularly impressive performance in challenging night conditions, where the environment exhibits greater complexity. By effectively capturing the multiple modes inherent in the error data, our approach significantly enhances localization accuracy under such circumstances.

 \setlength{\tabcolsep}{2.5pt}
\begin{table}[!bt]
\centering
\caption{Study case: evaluation results of Gaussian Sum Filter localization where 5.0\% / 4.7\% / 4.6\% of data are corrupted with average blurring.}
\label{table:eval_GSM_avgblurring}
\begin{tabular}{cl@{\hskip 0.15in}c@{\hskip 0.5in}c@{\hskip 0.45in}cc}
\toprule
Row & Method & Sunny & Night & Snowy \\ 
\midrule 
\multicolumn{5}{c}{Average measurement error: 108.21m/121.37m/108.66m.} \\

\midrule
1 & Constant Noise & 107.16 & 121.37 & 108.08 \\
2 & Constant Gaussian Mixture & 120.70 & 107.19 & 109.64 \\ 
3 & SPF & 3.37 & 7.70 & 3.35 \\ \midrule
4 & GSF & \textbf{2.83} & \textbf{4.13} &  \textbf{3.29} \\
\bottomrule
\end{tabular}
\end{table}


 \setlength{\tabcolsep}{2.5pt}
\begin{table}[!bt]
\centering
\caption{Study case: evaluation results of Gaussian Sum Filter localization where 5.0\% / 4.7\% / 4.6\% of data are corrupted with salt and pepper noise.}
\label{table:eval_GSM_snp0.5}
\begin{tabular}{cl@{\hskip 0.15in}c@{\hskip 0.5in}c@{\hskip 0.45in}cc}
\toprule
Row & Method & Sunny & Night & Snowy \\ 
\midrule 
\multicolumn{5}{c}{Average measurement error: 66.09m/103.63m/85.26m.} \\

\midrule
1 & Constant Noise & 65.36 & 102.88 & 84.73 \\
2 & Constant Gaussian Mixture & 74.36 & 87.01 & 84.55 \\ 
3 & SPF & 1.97 & 7.08 & \textbf{2.46} \\ \midrule
4 & GSF & \textbf{1.44} & \textbf{3.59} &  2.55 \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure}[htb]
  \centering
  \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/chapter5/analysis_1a.png}
    \caption{Single Gaussian}
    \label{fig:analysis_gmma}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/chapter5/analysis_1b.png}
    \caption{Gaussian Mixture}
    \label{fig:analysis_gmmb}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/chapter5/analysis_1c.png}
     \caption{Gaussian Mixture}
    \label{fig:analysis_gmmc}
  \end{subfigure}

    \caption{\small Comparison between an oversized single Gaussian and Gaussian Mixtures for representing measurement uncertainty. The left figure illustrates measurement uncertainty represented by a single Gaussian, which is oversized. The right two figures depict Gaussian mixtures used to represent the uncertainty of the same measurement. In the Gaussian mixtures, lighter colors indicate lower weights assigned to the mixture components.}
      \label{fig:analysis_gmm}
\end{figure}
Additionaly, we analyze the reasons behind the superior performance achieved by our proposed approach. Firstly, Gaussian Mixture Models offer a higher degree of flexibility in modeling complex distributions, which is essential when a single Gaussian distribution fails to adequately capture the distribution of the error data. This flexibility allows us to effectively represent the intricate patterns present in the data. Secondly, previous methods tend to ignore some measurements of good quality due to the oversized single Gaussian representation of uncertainty as shown in Figure \ref{fig:analysis_gmma}. However, by incorporating Gaussian Mixture Models, we can leverage the potential of these measurements. In our Gaussian Sum Filter, we assign a high weight to these measurements based on their likelihood, ensuring their significant influence in the filtering process, as shown in Figure \ref{fig:analysis_gmmb} and Figure \ref{fig:analysis_gmmc}. Consequently, our approach exhibits improved stability and accuracy, as it effectively utilizes all available information.


\begin{figure}[htbp]
\vskip-5pt
        \centering
        \includegraphics[width=0.85\linewidth]{figures/chapter5/Average Localization Error VS Number of GMM Components.png}
        \caption{\small Average localization error VS Number of GMM components.
        \label{fig:componentsVSperformance}}
        \vskip-5pt
\end{figure}
Finally, we demonstrate the correlation between the utilization of components in Gaussian Mixture Models and the effectiveness of localization, as illustrated in Figure \ref{fig:componentsVSperformance}. Our analysis reveals that a mere 2 components suffice to adequately account for uncertainty in both sunny and snowy conditions. However, in more intricate night conditions, 3 components of GMM prove to be adequate. Furthermore, these findings align consistently with the outcomes presented in Figure \ref{fig:bic_plot}.






==> sections/method.dump.tex <==
% We first give a brief overview of the visual localization pipeline\footnote{We focus on the image retrieval and matching part of the method and omit the 3D-structure based pose estimation which requires building complex 3D model} from~\cite{8953492}. Let $X=\{k_i\}_{i=1}^N$ be a set of database images where we know the GPS location of each image $x(k_i)$. Given a query image $q$, our goal is to estimate the location where image $q$ was taken from. To simplify the problem, we find the \textit{closest} image $f_\text{closest}(q;X)$ from the database $X$, and use its corresponding location as the predicted location $\hat{x}=x(f_\text{closest}(q;X))$.  

% The \textit{closest} image is defined as image with the most number of keypoint matches; more specifically, for each query image, we must perform keypoint matching with all $N$ database images. However, keypoint matching is computationally expensive. Thus, we utilize a global feature matching network (NetVLAD \cite{7780941}), that is computationally much faster, to retrieve top $n<<N$ candidate images from the database. Then, we perform keypoint matching only between the query and this smaller subset of database images. We use SuperPoint\cite{superpoint} for keypoint detection and SuperGlue~\cite{superglue} for keypoint matching. Note that the computation of global features and keypoint detection on the database images can be done in advance to save runtime.

% However, different from typical visual localization pipeline, we propose to use multiple databases from multiple traversals motivated by several key observations. First, more traversals makes the database denser and lowers the minimal location error between the closest image and the query image. Second, as the query image for localization can originate from different weather and lighting conditions, it is important to diversify the database images in order to reduce potential errors (those from the traversal and from keypoint mismatches). Finally and most importantly, data from multiple traversals can be used to provide a localization uncertainty prediction, as will be shown in \ref{sec:uncertainty_pred}. 

% Thus, we propose to use multiple traversals $X^1, X^2, \dots$ as one combined (large) database. But there is one problem that the retrieved candidate images may predominantly come from one same traversal because the appearance of query image is very similar to this traversal images, such as the example in \autoref{fig:example}, which mitigates the original goal of diversifying the database to lower the error. Therefore, instead of mixing different traversals, we retrieve candidates from each traversal and choose the image with most keypoint matches as shown in \autoref{fig:vislocpipeline}. 

==> sections/new_method.tex <==
 \begin{figure*}[t!]
        \centering
        \includegraphics[width=0.9\textwidth]{figures/pipeline_VL_v2.pdf}
        \caption{\small Pipeline for location prediction form image-retrieval using multiple traversals.
        \label{fig:vislocpipeline}}
        \vskip-15pt
\end{figure*}
\section{Method}\label{sec:method}
\subsection{Uncertainty Quantification From Repeated Information/ Data}\label{sec:uncertainty_pred}
\subsubsection{Problem Definition} 
Let $M:q\rightarrow r$ be a prediction model that takes input $q$ and predict $r\in \mathbb{R}^{n}$. We formally define uncertainty quantification of $r$ as estimating the error bound $\sigma_c(q)\in \mathbb{R}^{+}$ and confidence level $c\in [0,1]$ such that the error between the prediction $\hat{r}$ and the ground-truth $r_{\text{gt}}$ is below $\sigma_c$ by $c$ confidence (probability):
\begin{equation}
    p\left(\lVert \hat{r}-r_{\text{gt}} \rVert < \sigma_c(q) \right) = c
\end{equation}
%=================================================
\subsubsection{Uncertainty Modeling}
We propose to tackle this problem by creating an uncertainty model that maps key attributes/ signals of prediction to error bound $\sigma_c$ and confidence $c$ estimates.
For example, the error of stereo depth sensor is quadratic to range \cite{gallup2008variable}.
We propose to leverage repeated data (\eg multiple traversals passing the same route for autonomous driving data) to create the uncertainty model. Suppose we have $L>1$ dataset $X^1$ to $X^L$, we propose to do cross-validation. Specifically, we evaluate the prediction result on dataset $X^l$ using prediction model $M$ that \emph{learns} from another dataset $X^{m\neq l}$.

%JMJMJMJMJMJMJMJMJMJMJMJMJMJMJMJMJMJM
\color{green}CONTINUE HERE!!!!!\color{black}
A key component of our approach to uncertainty modeling is creating the sensor error model for each database/traversal, shown in \autoref{fig:pipeline} Top. To make the error model for a database $l$, we apply the image retrieval pipeline using traversal $X^l$ as the query and another traversal $X^{m\neq l}$ as the database. Specifically, for every image $k_i^l \in X^l$, we find the closest image $f(k_i^l; X^m)$ from database $m$ and compute their location error $\lVert x(f(k_i^l; X^m)) - x(k_i^l) \rVert$. Thus, for each image, we can compute the number of keypoint matches (to its closest image) and location error. This process is repeated using all $L-1$ different traversals as the database to obtain a list of number of keypoint matches and location errors.
We divide the data (number of keypoints vs error) into  bins according to the number of keypoint matches (\eg, bin 1 contains data points whose number of keypoint matches range from 0 to 200, bin 2 from 200 to 400, and so on).
For each bin, we empirically determine the error bound $\sigma_c$ for confidence $c$ such that $c$ fraction of data in that bin has smaller error than $\sigma_c$. We can create sensor error models for other traversals/ databases in the same way.


We first analyze the performance of the neural network predictions as a function of the number of keypoint matches $n_\text{kpm}$ by performing cross-validation using different databases. 
\autoref{fig:motivation3} shows two scatter plots of the location error between images from two databases (sunny and night) and their closest images from \emph{another} database (sunny) as a function of the number of keypoint matches.
    
We learn two things. First, the number of keypoint matches $n_\text{kpm}$ can serve as a good indicator for uncertainty quantification. Second, the relationship between number of keypoint matches versus error can be different for different databases (traversals); notice that the scatter plots for different databases in \autoref{fig:motivation3} have different distributions.
Thus, we propose to build the sensor error model as a function of number of  keypoint matches, and build one model for each different traversal. We can utilize multiple traversals to learn this mapping as follows. 
\begin{figure}[htbp]
\vskip-8pt
        \centering
        \includegraphics[width=1\linewidth]{figures/motivation/nkp_motivation.png}
        \caption{\small Relationship between number of keypoint matches and location error for two different database traversals.}
        \label{fig:motivation3}
        \vskip-8pt
\end{figure} 

 \begin{figure*}[htbp]
        \centering
        \includegraphics[width=0.9\textwidth]{figures/pipeline_v2.pdf}
        \caption{\small Pipeline for uncertainty prediction. Top: sensor error model calibration. Bottom: using sensor error model in inference. 
        \label{fig:pipeline}}
        \vskip-15pt
\end{figure*}

\subsubsection{Using Sensor Error Model to Predict Uncertainty}
The inference process is shown in \autoref{fig:pipeline} Bottom. Given a query image of unknown location, we predict the location, \ie, retrieve the closest image (as explained in \autoref{sec:visloc}); the location of the closest image becomes the predicted location.
If the closest image is from database $l$ ($X^l$), we refer to the corresponding sensor error model for database $l$. 
We find the bin associated with the number of keypoint matches (between query and closest image) and read the error bound $\sigma_c$ for confidence level $c$ that we target.

%=================================================
%*******************************************************************************************************************************************************************************************************************************************
\color{blue}
\subsection{Location Prediction from Image Retrieval}\label{sec:visloc}
We first start from a standard \emph{location prediction from image retrieval pipeline}\footnote{We focus on the image retrieval part of the method and omit the 3D-structure-based pose estimation, which requires building a complex 3D model.}~\cite{8953492}. 
Let $X=\{k_i\}_{i=1}^N$ be a set of database images with know GPS locations $r(k_i)$.
Given a query image $q$, our goal is to estimate the location where the image was taken from.
As images taken from close-by poses should preserve some content similarity, we find the \emph{closest} image $f_\text{closest}(q;X)$ from database $X$ and use its corresponding location as the predicted location $\hat{r}(q)=r(f_\text{closest}(q;X))$. 
We define the \emph{closest} image as the image with the most number of keypoint matches $n_\text{kpm}$ to the query image.
However, performing keypoint matching of the query image to all $N$ database images is very computationally expensive. Therefore, keypoint matching (SuperPoint\cite{superpoint} followed with SuperGlue~\cite{superglue}) is performed only on top $n<<N$ candidate images retrieved by global feature matching (NetVLAD~\cite{7780941}) that is computationally much faster.

A standard location prediction from image retrieval pipeline typically uses database from just one traversal (passing the route once).
We propose to use \emph{multiple databases} coming from multiple traversals motivated by several key observations. A query image has a non-zero distance to even its closest image from database (see \autoref{fig:motivation1}). 
Using multiple traversals increases the database image option to search from and lower the  minimum theoretical error. 
Second, as the query image for localization can originate from different weather and lighting conditions, it is important to diversify the database images to reduce potential errors (those from the traversal and from keypoint mismatches). Finally and most importantly, data from multiple traversals can be used to provide a localization uncertainty prediction, as will be shown in \ref{sec:uncertainty_pred}.

One naive approach of using more data is to simply treat the additional data from multiple traversals $X^1, X^2, \dots, X^L$ as one combined (large) database and just apply the same standard pipeline. However, this is not effective, as the candidate images retrieved by global feature matching may predominantly come from a single database whose color tone or even foreground object appearance is most similar to the query image, hindering the original goal of diversifying the database to lower the error. 
This motivates a new approach to encourage retrieval of candidate images from \textit{every single} traversal as shown in \autoref{fig:vislocpipeline}.
\begin{figure}[htbp]
        \vskip-8pt
        \centering
        \includegraphics[width=0.7\linewidth]{figures/motivation/multipletraj.png}
        \caption{\small GPS locations of several traversals (zoomed in for illustration; full trajectory is not shown). Using multiple traversals increases the chances that a database image is closer to the query image location (\ie, smaller theoretical error).
        \label{fig:motivation1}}
        \vskip-10pt
\end{figure}
%===============================================================
\subsection{Full Visual Localization Pipeline}\label{sec:method-filter}
We take the output of the location prediction (\autoref{sec:visloc})  as \textit{uncertain sensor measurements} in our Sigma Point (Unscented) filter (SPF) localization framework \cite{wan2000unscented,Brunke2004}. Our goal is to estimate the probability $p(s_t|m_{1:t})$ of the state vector $s_t$ at time $t$ given observed measurements $m_{1:t}$ from time $1$ to $t$.
We define the state vector as follows:
\begin{equation}
    s = \begin{bmatrix}x & y & \theta & v & \dot{\theta} \end{bmatrix}^T
\end{equation}
, where $x,y,\theta$ are the planar position and heading angle, while $v, \dot{\theta}$ are the linear and angular velocity of the car. In the prediction step of the SPF, we assume constant linear and angular velocity ($v$ and $\dot{\theta}$) and follow the standard prediction step of SPF~\cite{wan2000unscented}. 
In the measurement update, given an image input, we process the image through the location and uncertainty prediction pipeline (\ref{sec:visloc} and \ref{sec:uncertainty_pred}) and take their output as the measurement. 
Specifically, the measurement vector takes the predicted $x$ and $y$ location from \autoref{sec:visloc}.
We adapt \ref{sec:uncertainty_pred} to form the measurement covariance matrix. Specifically, we compute the measurement covariance $R \in \mathbb{R}^{2\times 2}$ from the cross-validation data, per database, per number of keypoint matches range (bin). The covariance matrices are formed and expressed in the ego car coordinate and transformed to the world coordinate during inference/ filter.
%We utilize the uncertainty prediction from \ref{sec:uncertainty_pred} to construct the measurement covariance:
%\begin{equation}
%    R = \begin{bmatrix} \sigma_{x_{VL}}^2 & 0 \\
%    0 & \sigma_{y_{VL}}^2
%    \end{bmatrix}
%\end{equation}
%For every image measurement $q$, we refer the corresponding sensor error model and retrieve $\sigma_c(q)$ at $c=68\%$ for one Gaussian standard deviation, and use $\sigma_x=\sigma_y=\sigma_{68\%}(q)$.
Note that different measurements may result in different covariance (due to reading different sensor error model, as well as referring to different bin in a model).
Given the measurement vector and its covariance, the measurement update then simply follows the SPF measurement update in \cite{wan2000unscented}.

Estimation framework typically also employs \textit{sensor measurement gating} to decide whether to accept (use it in the measurement update) or reject measurements. This is similar to \textit{outlier rejection} of the sensor measurement. Given a measurement vector $m$, we compute the Mahalanobis distance $d_M$ defined as follows:
\begin{equation}
    d_M^2 = (m-\hat{m})^T (H\hat{C}H^T+R)^{-1} (m-\hat{m})
\end{equation}
, where $\hat{C}$ is the estimated state covariance$, \hat{m}$ is the expected measurement, and $H$ is the measurement matrix that maps the state vector to the measurement.
The measurement is rejected if it lies outside of the validation gate, 
%\ie the squared of Mahalanobis distance  $d_M^2$ is greater than a certain threshold $\chi^2_{k,\alpha}$: 
\begin{equation}\label{eq:chi2}
    \text{if } d_M^2 > \chi^2_{k,\alpha} \rightarrow \text{reject},
\end{equation}
where $\chi^2_{k,\alpha}$ is taken from the inverse chi-squared $\chi^2$ cumulative distribution at a level $\alpha$ with $k$ degree of freedom. The level $\alpha$ controls the validation gate, \ie it rejects $(1-\alpha)\times 100\%$ of the measurements at the tail. Typical values of $\alpha$ are $0.99$, $0.975$, and $0.95$.
%For example, for a two-dimensional measurement vector ($k=2$), to reject $1\%$ tail of the measurement ($\alpha=1-0.01=0.99$), a threshold of $\gamma=9.2$ will reject $1\%$ of the tail.
% Refer to Brian's tree paper for inspiration on writing this section https://arxiv.org/pdf/2103.15967.pdf
% also to my paper, to see how to write notations for filter etc
% Some ref for gating: http://ais.informatik.uni-freiburg.de/teaching/ws11/robotics2/pdfs/rob2-20-dataassociation.pdf
\color{black}


==> sections/related_works.tex <==
\section{Related Works}
\label{sec:related_works}
%=======================================================
\subsection{Uncertainty Modeling.} 
%Bayesian neural networks~\cite{10.1162/neco.1992.4.3.448,10.5555/525544} estimate the uncertainty by regarding weights in networks as random variables instead of true constant values. 
Bayesian neural networks (BNN)~\cite{10.1162/neco.1992.4.3.448,10.5555/525544} estimate uncertainties by treating neural network weights as random variables.
Predictions are in the form of an expectation with respect to the posterior distribution over the model weights. Two prominent methods for approximate inference in BNNs are Bayes by Backprop~\cite{blundell2015weight} and Monte Carlo (MC) dropout~\cite{gal2016dropout}. Bayes by Backprop regularises the weights by minimising the expected lower bound on the marginal likelihood. MC Dropout interprets dropout approximately as integrates over the models’ weights. However, specifying a meaningful prior for the parameters can be challenging. More over, the uncertainty is often poorly calibrated. Another popular approach for neural network uncertainty estimation is ensemble method~\cite{10.5555/3295222.3295387,ValdenegroToro2019DeepSF,Wen2020BatchEnsembleAA}. Ensemble methods train multiple different networks and combine their predictions to make a final prediction. The uncertainty is represented by the variance of these predictions. Our approach differs from these approaches in the way that our approach does not change the neural network structure and can be applied to any network.  

% \color{red}Bayes by Backprop regularises the weights by minimising the expected lower bound on the marginal likelihood. MC Dropout builds a probabilistic interpretation of dropout which allows model uncertainty to be obtained from existing deep learning models. However, BNNs heavily rely on a strong assumption of independence between parameters. Computational complexity of approximate inference is reduced but at the cost of probabilistic accuracy~\cite{Goan_2020}. 
% Ensemble of networks includes several neural networks of different parameter
% settings. The results will be determined by combining outputs of these neural networks with different settings. Our approach differs from these approaches in the way that our approach does not change the neural network structure and has potential to be applied to any pre-trained network. \color{black}

Another line of work for uncertainty estimation is post-processing methods~\cite{guo2017calibration,07998,pmlr-v80-kuleshov18a}, which are applied after the training process of neural networks. 
%These approaches aim at learning a calibration function by different ways. 
\cite{guo2017calibration} compares different calibration methods and show that temperature scaling is the simplest, fastest, and often most effective of these methods. Inspired by classification calibration techniques, \cite{pmlr-v80-kuleshov18a} extends to regression tasks and outputs well calibrated results on regression networks. However, these methods either require inputs of uncalibrated uncertainty or re-training some layers. 
Our method is inspired by these methods but differs in the way that our method predicts well-calibrated uncertainty without inputs of uncalibrated uncertainty or re-traininig. It is possible to combine them together.   

%=============================================
\subsection{Visual Localization} 
Visual localization infers the pose of the query images by utilizing information from the surrounding environment, such as images and point clouds. Two main branches of visual localization are image-based localization and 3D-structure-based localization. 
Image-based localization~\cite{6248018,7410496,Radenovi2016CNNIR} can be understood as an image retrieval problem, \ie retrieving the most similar image from a database/library of images with known poses, taking the pose of the retrieved image as the predicted pose.
For example, DenseVLAD~\cite{7298790} finds the closest image based on the distance of densely sampled SIFT descriptors across multiple scales. Different from DenseVLAD, NetVLAD~\cite{7780941} learns the descriptor by combining the vector of locally aggregated descriptors with CNN. 
 Although 2D-image-based approaches is generally less accurate than 3D-structure based localization, but it is more simple and robust to environmental change~\cite{Xin2019ARO}. 
%3D-structure-based localization~\cite{Irschara,8578819,Geppert,Nadeem,Germain,Sattler} requires having a 3D model or map along with an image database/library. It uses both image and 3D point cloud measurement to estimate the pose. Specifically, it finds the pose that gives the best matching between the detected 2D keypoints in the query image and 3D keypoints in the preconstructed 3D model. \cite{8953492} also propose a hierarchical fashion combining 2D image retrieval with 3D-structure based approaches. In this hierarchical settings, NetVLAD~\cite{7780941} retrieves several candidate images first. Then SuperPoint~\cite{superpoint} detects keypoints in images by self-supervised training with incorporating homographic adaptation and SuperGlue~\cite{superglue} learns keypoint matching through a graph neural network and attention mechanism. Comparing to 2D-image-based approaches, 3D-structure based localization can generally achieve a better accuracy but at the cost of poor performance in
terms of environmental change robustness~\cite{Xin2019ARO}. 

%**************************************************************************************
%Thus, how to achieve a good performance for keypoint detection and matching is of vital importance. Among these state-of-the-art approaches, SuperPoint~\cite{superpoint} detects keypoints in images by self-supervised training with incorporating homographic adaptation. SuperGlue~\cite{superglue} learns keypoint matching through a graph neural network and attention mechanism. The two approaches show a good performance for the two tasks. 



% \color{red}
% SuperPoint~\cite{superpoint} enables self-supervised training of image keypoint detection by using homographic adaptation. SuperGlue~\cite{superglue} uses a graph neural network and attention mechanism to learn keypoint matching.  

% \color{black}
%Some works~\cite{Germain,Sattler,8953492} also propose a hierarchical fashion combining 2D image retrieval with 3D-structure based approaches. Comparing to 2D-image-based approaches, 3D-structure based localization can generally achieve a better accuracy but at the cost of poor performance in
%terms of environmental change robustness~\cite{Xin2019ARO}.  %%Although the accuracy is generally inferior to 3D-structure-based approaches, image-based localization is fast, simple, and robust.

%%In this work, instead of building a state-of-the-art visual localization model, our focus is on uncertainty modeling with the application in visual localization, where we start with pipeline of~\cite{8953492} as a baseline\JC{baseline ?}. 


==> tables/dataset_info.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Dataset information for database ($X^1$, \dots, $X^{9}$) and query/ test ($Q^\text{sunny}$, $Q^\text{night}$, and $Q^\text{snow}$) traversals .}
\label{table:dataset_info}
\begin{tabular}{cccccccc}
\toprule
Traversal & $X^{1}$ & $X^{2}$ & $X^{3}$ & $X^{4}$ & $X^{5}$ & $X^{6}$ & $X^7$  \\ 
\midrule
Condition  & sunny & sunny& sunny & night & night & night & snowy   \\
\#images  & 12053
 & 13615 & 13496 & 14482 &  15370   & 15633 &  14542 \\
\bottomrule
\end{tabular}

\vspace*{1em}

\begin{tabular}{cccccc}
\toprule
Traversal &  $X^{8}$&$X^{9}$ &  $Q^\text{sunny}$ & $Q^\text{night}$ & $Q^\text{snow}$  \\ 
\midrule
Condition & snowy & snowy & sunny & night & snowy   \\
\#images& 13398 & 14186 & 9939 &  10614 & 10786  \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}




==> tables/eval_UKF_car.tex <==
 \setlength{\tabcolsep}{2.5pt}
\begin{table*}[!bt]
%\begin{table}[h]
\centering
\begin{center}
\caption{Evaluation result of Kalman Filter localization for \cone{sunny}, \ctwo{night}, and \cthree{snowy} conditions.}
\label{table:eval_UKF_car}
%\resizebox{\textwidth}{!}{
\begin{tabular}{clc@{\hskip 0.02in}ccc@{\hskip 0.06in}ccc@{\hskip 0.06in}ccc}
\toprule
Row & Method & Gating $(1-\alpha)$ & \cone{$d_\text{err}$(m) $\downarrow$}& \cone{Cov-credibility(\%)} & \cone{$n_r(\%)$} & \ctwo{$d_\text{err}$(m) $\downarrow$} & \ctwo{Cov-credibility(\%)} & \ctwo{$n_r(\%)$} & \cthree{$d_\text{err}$(m) $\downarrow$} & \cthree{Cov-credibility(\%)} & \cthree{$n_r(\%)$}\\ \midrule 
%\multicolumn{12}{c}{Normal measurement --- Average measurement error: \cone{0.83m,0.87m,0.87m} / \ctwo{11.67m ,8.68m,8.68m} / \cthree{1.76m,1.42m,1.42m}}
\multicolumn{12}{c}{Normal measurement --- Average measurement error: \cone{0.83m} / \ctwo{11.67m} / \cthree{1.76m} for MC dropout -- \cone{0.87m} / \ctwo{8.68m} / \cthree{1.42m} for baseline and ours.}
\\
\midrule
1 & MC d.o & 0 & \cone{0.79} & \cone{32.8 / 67.4 / 84.7} & \cone{0} & \ctwo{7.44} & \ctwo{27.6 / 56.2 / 71.0} & \ctwo{0} & \cthree{1.50} & \cthree{20.4 / 50.4 / 69.8} & \cthree{0}\\
2 & Baseline+SPF & 0 & \cone{0.76} & \cone{46.1 / 81.2 / 92.3} & \cone{0} & \ctwo{8.42} & \ctwo{38.5 / 67.0 / 78.9} & \ctwo{0} & \cthree{1.30} & \cthree{30.5 / 61.8 / 79.6} & \cthree{0}\\
3 & Gaussian+SPF     & 0 & \cone{0.57} & \cone{62.2 / 91.4 / 97.4} & \cone{0} & \ctwo{3.07} & \ctwo{75.9 / \textbf{94.6} / \textbf{98.6}} & \ctwo{0} & \cthree{\textbf{0.81}} & \cthree{55.4 / 86.4 / 95.9} & \cthree{0}\\ 
4 & Baseline+GSF     & 0 & \cone{1.06} & \cone{97.3 / 99.0 / \textbf{99.2}} & \cone{0} & \ctwo{1.13} & \ctwo{\textbf{66.8} / 88.8 / 96.2} & \ctwo{0} & \cthree{1.21} & \cthree{52.3 / 82.7 / 94.2} & \cthree{0}\\
5 & GMM+GSF     & 0 & \cone{\textbf{0.57}} & \cone{\textbf{70.7} / \textbf{93.4} / 98.5} & \cone{0} & \ctwo{\textbf{1.09}} & \ctwo{73.9 / 93.9 / 98.5} & \ctwo{0} & \cthree{0.84} & \cthree{\textbf{61.8} / \textbf{88.1} / \textbf{96.8}} & \cthree{0}\\
\midrule
4 & MC d.o & 1.0\% & \cone{0.612} & \cone{33.1 / 68.2 / 85.6} & \cone{1.0} & \ctwo{165.282} & \ctwo{23.4 / 46.0 / 57.7} & \ctwo{33.0} & \cthree{\textbf{1.442}} & \cthree{21.2 / 51.6 / \textbf{71.6}} & \cthree{4.8}\\
5 & Baseline & 1.0\% & \cone{0.610} & \cone{46.6 / 82.1 / 93.3} & \cone{1.0} & \ctwo{54.382} & \ctwo{33.9 / 57.2 / 67.0} & \ctwo{30.3} & \cthree{333.538} & \cthree{17.5 / 38.3 / 51.7} & \cthree{37.7}\\
6 & Ours     & 1.0\% & \cone{\textbf{0.570}} & \cone{\textbf{62.3} / \textbf{91.4} / \textbf{97.5}} & \cone{0.2}  & \ctwo{\textbf{2.926}} & \ctwo{\textbf{76.2} / \textbf{94.6} / \textbf{98.7}} & \ctwo{0.3} & \cthree{222.608} & \cthree{\textbf{34.5} / \textbf{56.4} / 63.9} & \cthree{33.2}\\ 
\midrule
7 & MC d.o & 2.5\% & \cone{\textbf{0.613}} & \cone{33.1 / \textbf{68.2} / \textbf{85.9}} & \cone{1.5} & \ctwo{7607.294} & \ctwo{3.6 / 8.5 / 11.5} & \ctwo{86.7} & \cthree{8144.861} & \cthree{3.7 / 9.0 / 12.3} & \cthree{82.5}\\
8 & Baseline & 2.5\% & \cone{790.307} & \cone{32.8 / 54.5 / 61.6} & \cone{35.2} & \ctwo{54.205} & \ctwo{34.1 / 57.9 / 69.1} & \ctwo{31.3} & \cthree{8169.233} & \cthree{5.1 / 11.2 / 14.8} & \cthree{82.3}\\
9 & Ours     & 2.5\% & \cone{82.828} & \cone{\textbf{47.7} / 67.9 / 72.5} & \cone{26.2} & \ctwo{\textbf{2.942}} & \ctwo{\textbf{76.3} / \textbf{94.6} / \textbf{98.7}} & \ctwo{0.4} & \cthree{\textbf{8121.261}} & \cthree{\textbf{7.6} / \textbf{14.1} / \textbf{16.7}} & \cthree{82.0}\\
%=======================================================================================================================================
\midrule
\multicolumn{12}{c}{Study case where \cone{5.0\%} / \ctwo{4.7\%} / \cthree{4.6\%} of data are  corrupted with average blurring --- Average measurement error: \cone{108.21m} / \ctwo{121.78m} / \cthree{108.66m}}\\
\midrule
10 & Baseline+SPF & 0 & \cone{107.16} & \cone{41.9 / 74.6 / 85.4} & \cone{0} & \ctwo{121.37} & \ctwo{36.3 / 63.5 / 74.4} & \ctwo{0} & \cthree{108.08} & \cthree{29.2 / 58.9 / 75.3} & \cthree{0}\\
11 & Gaussian+SPF     & 0 & \cone{3.37} & \cone{61.0 / 90.3 /  96.9} & \cone{0} & \ctwo{7.70} & \ctwo{\textbf{72.9} / 92.7 / 97.2} & \ctwo{0} & \cthree{3.35} & \cthree{56.4 / 87.0 / 95.7} & \cthree{0}\\ 
12 & Baseline+GSF     & 0 & \cone{120.70} & \cone{86.1 / 88.2 /  89.3} & \cone{0} & \ctwo{107.19} & \ctwo{44.6 / 60.4 / 68.3} & \ctwo{0} & \cthree{109.64} & \cthree{49.5 / 77.3 / 87.5} & \cthree{0}\\
13 & GMM+GSF     & 0 & \cone{\bf{2.83}} & \cone{\bf{70.0} / \bf{92.2} / \bf{98.2}} & \cone{0} & \ctwo{\textbf{4.13}} & \ctwo{75.4 / \bf{93.0} / \bf{97.7}} & \ctwo{0} & \cthree{\textbf{3.29}} & \cthree{\textbf{63.2} / \textbf{88.3} / \textbf{96.5}} & \cthree{0}\\ 
\midrule
12 & Baseline & 1.0\% & \cone{1726.025} & \cone{3.6 / 7.1 / 8.3} & \cone{91.1} & \ctwo{8776.021} & \ctwo{1.8 / 2.6 / 3.4} & \ctwo{97.2} & \cthree{726.828} & \cthree{14.9 / 28.9 / 37.0} & \cthree{58.7}\\
13 & Ours     & 1.0\% & \cone{\textbf{3.529}} & \cone{\textbf{61.3} / \textbf{90.6} / \textbf{97.0}} & \cone{1.3} & \ctwo{\textbf{66.813}} & \ctwo{\textbf{65.8} / \textbf{82.3}/ \textbf{86.7}} & \ctwo{12.4} & \cthree{\textbf{264.000}} & \cthree{\textbf{35.8} / \textbf{57.4} / \textbf{64.2}} & \cthree{33.3}\\ \midrule
14 & Baseline & 2.5\% & \cone{1756.856} & \cone{6.0 / 8.0 / 8.9} & \cone{91.4} & \ctwo{1510.11} & \ctwo{6.0 / 11.4 / 15.6} & \ctwo{84.1} & \cthree{8169.514} & \cthree{5.5 / 11.6 / 15.0} &	\cthree{83.3}\\
15 & Ours     & 2.5\% & \cone{\textbf{110.299}} & \cone{\textbf{51.3} / \textbf{73.2} / \textbf{78.2}} & \cone{20.6} & \ctwo{\textbf{70.659}} & \ctwo{\textbf{65.9} / \textbf{82.0} / \textbf{86.5}} & \ctwo{13.2} & \cthree{\textbf{820.152}} & \cthree{\textbf{16.0} / \textbf{29.0} / \textbf{34.8}} &	\cthree{62.1}\\
%=======================================================================================================================================
\midrule
\multicolumn{12}{c}{Study case where \cone{5.0\%} / \ctwo{4.7\%} / \cthree{4.6\%} of data are corrupted with salt and pepper noise --- Average measurement error:  \cone{66.09m} / \ctwo{103.63m} / \cthree{85.26m}}\\
\midrule
16 & Baseline+SPF & 0 & \cone{65.36} & \cone{42.0 / 74.9 / 85.6} & \cone{0} & \ctwo{102.88} & \ctwo{36.8 / 63.9 / 75.0} & \ctwo{0} & \cthree{84.73} & \cthree{29.1 / 58.7 / 75.1} & \cthree{0}\\
17 & Gaussian+SPF    & 0 & \cone{1.97} & \cone{61.9 / 91.1 / 97.4} & \cone{0} & \ctwo{7.08} & \ctwo{\textbf{73.1} / 92.2 / 97.1} & \ctwo{0} & \cthree{\textbf{2.46}} & \cthree{57.0 / 87.4 / 96.1} & \cthree{0}\\ 
18 & Baseline+GSF     & 0 & \cone{74.36} & \cone{88.1 / 89.7 / 90.1} & \cone{0} & \ctwo{87.01} & \ctwo{42.7 / 62.1 / 72.6} & \ctwo{0} & \cthree{84.55} & \cthree{49.6 / 77.4 / 87.7} & \cthree{0}\\
19 & GMM+GSF     & 0 & \cone{\bf{1.44}} & \cone{\bf{69.9} / \bf{92.3} / \bf{98.0}} & \cone{0} & \ctwo{\textbf{3.59}} & \ctwo{75.5 / \bf{93.1} / \bf{98.1}} & \ctwo{0} & \cthree{2.55} & \cthree{\textbf{63.3} / \textbf{88.7} / \textbf{97.0}} & \cthree{0}\\ 
\midrule
18 & Baseline & 1.0\% & \cone{\bf{0.985}} & \cone{45.8 / 80.4 / 92.1} & \cone{5.5} & \ctwo{3563.210} & \ctwo{24.6 / 36.2 / 40.2} & \ctwo{60.4} & \cthree{\textbf{724.023}} & \cthree{\textbf{15.1} / \textbf{29.3} / \textbf{38.0}} & \cthree{56.7}\\
19 & Ours     & 1.0\% & \cone{1.719} & \cone{\textbf{62.3} /	\textbf{91.3} / \textbf{97.5}} & \cone{0.6} & \ctwo{\textbf{437.251}} & \ctwo{\textbf{28.7} / \textbf{40.6} / \textbf{48.0}} & \ctwo{39.5} & \cthree{1329.145} & \cthree{13.3 / 17.7 / 18.8} &	\cthree{76.7}\\ \midrule
20 & Baseline & 2.5\% & \cone{420.962} & \cone{35.2 / 58.2 / 66.7} & \cone{33.7} & \ctwo{1308.586} & \ctwo{2.2 / 3.2 / 7.9} & \ctwo{96.1} & \cthree{1554.474} & \cthree{2.2 / 3.8 / 6.4}	& \cthree{94.5}\\
21 & Ours     & 2.5\% & \cone{\textbf{81.392}} & \cone{\textbf{48.3} / \textbf{68.4} / \textbf{74.0}} & \cone{25.4} & \ctwo{\textbf{408.598}} & \ctwo{\textbf{27.6} / \textbf{38.7} / \textbf{46.6}} & \ctwo{42.8} & \cthree{\textbf{1110.267}} & \cthree{\textbf{7.4} / \textbf{13.4} / \textbf{17.6}} &	\cthree{79.9}\\


\bottomrule
\end{tabular}
%}
\end{center}
\vskip-10pt
\end{table*}
 \setlength{\tabcolsep}{1.4pt}



% ###################################################### plain version without formatting
% % \setlength{\tabcolsep}{4pt}
% \begin{table*}[h]
% %\begin{table}[h]
% \centering
% \begin{center}
% \caption{Evaluation result of Unscented Kalman Filter}
% \label{table:eval_UKF_car}
% %\resizebox{\textwidth}{!}{
% \begin{tabular}{c|c|ccc|ccc|ccc}
% \toprule
%  & Condition & \multicolumn{3}{c}{$Q^\text{sunny}$} & \multicolumn{3}{c}{$Q^\text{night}$} & \multicolumn{3}{c}{$Q^\text{snowy}$} \\
% \midrule
% Metric & Gating & $d_\text{err}$(m) & Cov-credibility(\%) & $n_r$ & $d_\text{err}$(m) & Cov-credibility(\%) & $n_r$ & $d_\text{err}$(m) & Cov-credibility(\%) & $n_r$\\
% \midrule
% Baseline & N/A & 0.766 & 46.1 / 81.2 / 92.3 & 0 & 8.425 & 38.5 / 67.0 / 78.9 & 0 & 1.302  & 30.5 / 61.8 / 79.6 & 0\\
% Ours     & N/A & 0.569 & 62.2 / 91.4 / 97.4 & 0 & 3.075 & \textbf{75.9} / 94.6 / 98.6 & 0 & \textbf{0.811} & \textbf{55.4} / \textbf{86.4} / \textbf{95.9} & 0\\
% Baseline & 1.0\% & 0.610 & 46.6 / 82.1 / 93.3 & 96 & 54.382 & 33.9 / 57.2 / 67.0 & 3221 & 333.538 & 17.5 / 38.3 / 51.7 & 4063\\
% Ours     & 1.0\% & \textbf{0.570} & \textbf{62.3} / \textbf{91.4} / \textbf{97.5} & 18 & \textbf{2.926} & 76.2 / \textbf{94.6} / \textbf{98.7} & 27	& 222.608 & 34.5 / 56.4 / 63.9 & 3577\\
% Baseline & 2.5\% & 790.307 & 32.8 / 54.5 / 61.6 & 3495 & 54.205 & 34.1 / 57.9 / 69.1	& 3322 & 8169.233 & 5.1 / 11.2 / 14.8 & 8872\\
% Ours     & 2.5\% & 82.828 &	47.7 / 67.9 / 72.5 & 2606 & 2.942 & 76.3 /  94.6 / 98.7 &	42 & 8121.261 & 7.6 / 14.1 / 16.7 &8849\\

% \midrule
% \multicolumn{11}{c}{ Study Case: Avg Blur 80 }\\
% \midrule
% Baseline & N/A & 107.163 & 41.9 / 74.6 / 85.4 & 0 & 121.370 & 36.3 / 63.5 / 74.4 & 0 & 108.080 & 29.2 / 58.9 / 75.3 & 0\\
% Ours     & N/A & \textbf{3.371} & 61.0 / 90.3 / 96.9 & 0 & \textbf{7.702} & 72.9 / \textbf{92.7} / \textbf{97.2} & 0 & \textbf{3.351} & \textbf{56.4} / \textbf{87.0} / \textbf{95.7} & 0\\
% Baseline & 1.0\% & 1726.025	& 3.6 / 7.1 / 8.3 & 9054 & 8776.021 & 1.8 / 2.6 / 3.4& 10312 & 726.828 & 14.9 / 28.9 / 37.0  & 6326\\
% Ours     & 1.0\% & 3.529 & \textbf{61.3} / \textbf{90.6} / \textbf{97.0} & 156 & 66.813 & \textbf{65.8} / 82.3 / 86.7 & 1317 & 264.000 & 35.8 / 57.4 / 64.2 & 3597\\
% Baseline & 2.5\% & 1756.856 & 6.0 / 8.0 / 8.9 & 9087 & 1510.11 & 6.0 / 11.4 / 15.6 & 8924 & 8169.514 & 5.5 / 11.6 / 15.0 &	8984\\
% Ours     & 2.5\% & 110.299 & 51.3 / 73.2 / 78.2 & 2049 & 70.659 & 65.9 / 82.0 / 86.5 & 1396 & 820.152 & 16.0 / 29.0 / 34.8 &	6698\\

% \midrule
% \multicolumn{11}{c}{Study Case: S\&P Noise 0.5} \\
% \midrule
% Baseline & N/A & 65.365 & 42.0 / 74.9 / 85.6 & 0 & 102.887 & 36.8 / 63.9 / 75.0 &		0 & 84.738 &	29.1 / 58.7 / 75.1 & 0\\
% Ours     & N/A & 1.971 & 61.9 / 91.1 / 97.4	 & 0 & \textbf{7.083} & \textbf{73.1} / \textbf{98.2} / \textbf{97.1} & 0 & \textbf{2.468} & \textbf{57.0} / \textbf{87.4} / \textbf{96.1} & 0\\
% Baseline & 1.0\% & \textbf{0.985} & 45.8 / 80.4 / 92.1 & 542 & 3563.210 & 24.6 / 36.2 / 40.2 &  6407 & 724.023 & 15.1 / 29.3 / 38.0 & 6114\\
% Ours     & 1.0\% & 1.719 & \textbf{62.3} / \textbf{91.3} / \textbf{97.5} & 57 & 437.251 & 28.7 / 40.6 / 48.0 &	4190 & 1329.145 & 13.3 / 17.7 / 18.8 & 8268\\
% Baseline & 2.5\% & 420.962 & 35.2 / 58.2 / 66.7 & 3351 & 1308.586 & 2.2 / 3.2 / 7.9	& 10200 & 1554.474 & 2.2 / 3.8 / 6.4 & 10197\\
% Ours     & 2.5\% & 81.392 & 48.3 / 68.4 / 74.0 & 2529 & 408.598 & 27.6 / 38.7 / 46.6	& 4538 & 1110.267 & 7.4 / 13.4 / 17.6 & 8613\\

% \bottomrule
% \end{tabular}
% %}
% \end{center}
% \end{table*}


==> tables/eval_UKF_world.tex <==
 \setlength{\tabcolsep}{3pt}
\begin{table*}[h]
%\begin{table}[h]
\centering
\begin{center}
\caption{Evaluation result of Unscented Kalman Filter localization for \cone{sunny}, \ctwo{night}, and \cthree{snowy} conditions.}
\label{table:eval_UKF_world}
%\resizebox{\textwidth}{!}{
\begin{tabular}{l c@{\hskip 0.2in}ccc@{\hskip 0.2in}ccc@{\hskip 0.2in}ccc}
\toprule
Method & Gating & \cone{$d_\text{err}$(m) $\downarrow$}& \cone{Cov-credibility(\%)} & \cone{$n_r(\%)$} & \ctwo{$d_\text{err}$(m) $\downarrow$} & \ctwo{Cov-credibility(\%)} & \ctwo{$n_r(\%)$} & \cthree{$d_\text{err}$(m) $\downarrow$} & \cthree{Cov-credibility(\%)} & \cthree{$n_r(\%)$}\\ \midrule 
\multicolumn{11}{c}{Normal measurement with average measurement error of \cone{0.87m} / \ctwo{8.68m} / \cthree{1.42m}}\\
\midrule
Baseline & 0 & \cone{0.782} & \cone{43.7 / 79.6 / 91.0} & \cone{0} & \ctwo{7.976} & \ctwo{37.2 / 63.8 / 74.7} & \ctwo{0} & \cthree{1.311} & \cthree{29.1 / 60.2 / 77.3} & \cthree{0}\\
Ours     & 0 & \cone{0.583} & \cone{64.6 / 92.5 / 97.6} & \cone{0} & \ctwo{2.796} & \ctwo{\textbf{78.3} / 95.1 / 98.6} & \ctwo{0} & \cthree{\textbf{0.826}} & \cthree{\textbf{60.8} / \textbf{88.9} / \textbf{96.4}} & \cthree{0}\\ \midrule
Baseline & 1.0\% & \cone{0.627} & \cone{44.3 / 80.7 / 92.3} & \cone{1.2} & \ctwo{207.580} & \ctwo{30.6 / 50.7 / 58.6} & \ctwo{4194} & \cthree{278.777} & \cthree{16.7 / 37.5 / 50.4} & \cthree{4118}\\
Ours     & 1.0\% & \cone{0.582} & \cone{64.7 / 92.6 / 97.8} & \cone{0.3}  & \ctwo{2.682} & \ctwo{78.7 / 95.3 / 98.7} & \ctwo{35} & \cthree{1.066} & \cthree{60.8 / 88.4 / 95.9} & \cthree{120}\\ 
\midrule
Baseline & 2.5\% & \cone{513.177} & \cone{31.1 / 53.8 / 61.5} & \cone{35.1} & \ctwo{197.811} & \ctwo{31.2 / 51.6 / 60.2} & \ctwo{4177} & \cthree{8123.550} & \cthree{5.1 / 11.1 / 14.5} & \cthree{8886}\\
Ours     & 2.5\% & \cone{\textbf{0.580}} & \cone{\textbf{64.8} / \textbf{92.7} / \textbf{97.9}} & \cone{0.5} & \ctwo{\textbf{2.681}} & \ctwo{78.8 / \textbf{95.4} / \textbf{98.8}} & \ctwo{51} & \cthree{8153.326} & \cthree{8.3 / 14.8 / 17.0} & \cthree{8854}\\
%=======================================================================================================================================
\midrule
\multicolumn{11}{c}{Study case (avg blur) with average measurement error of \cone{66.09m} / \ctwo{103.63m} / \cthree{85.26m}}\\
\midrule
Baseline & 0 & \cone{107.304} & \cone{39.8 / 73.2 / 84.1} & \cone{0} & \ctwo{120.329} & \ctwo{35.2 / 60.2 / 70.4} & \ctwo{0} & \cthree{108.067} & \cthree{27.8 / 57.0 / 72.6} & \cthree{0}\\
Ours     & 0 & \cone{\textbf{3.998}} & \cone{\textbf{63.5} / \textbf{90.9} / \textbf{96.5}} & \cone{0} & \ctwo{\textbf{8.534}} & \ctwo{\textbf{75.5} / \bf{92.8} / \bf{96.6}} & \ctwo{0} & \cthree{\textbf{3.674}} & \cthree{\textbf{61.4} / \textbf{88.5} / \textbf{95.7}} & \cthree{0}\\ \midrule
Baseline & 1.0\% & \cone{1887.397} & \cone{2.4 / 3.8 / 4.2} & \cone{99.0} & \ctwo{1148.243} & \ctwo{24.3 / 36.4 / 39.7} & \ctwo{6482} & \cthree{779.419} & \cthree{13.8 / 27.3 / 34.3} & \cthree{6665}\\
Ours     & 1.0\% & \cone{515.619} & \cone{44.1 / 61.6 / 65.0} & \cone{33.3} & \ctwo{9.643} & \ctwo{76.1 / 93.0/ 96.6} & \ctwo{190} & \cthree{103.057} & \cthree{48.7 / 73.3 / 80.3} & \cthree{1919}\\ \midrule
Baseline & 2.5\% & \cone{1755.166} & \cone{5.6 / 8.1 / 8.9} & \cone{91.4} & \ctwo{1781.440} & \ctwo{1.8 / 3.1 / 3.5} & \ctwo{10295} & \cthree{8123.241} & \cthree{5.3 / 11.4 / 14.7} &	\cthree{8984}\\
Ours     & 2.5\% & \cone{93.727} & \cone{48.4 / 68.0 / 72.5} & \cone{26.9} & \ctwo{10.514} & \ctwo{75.6 / 92.7 / 96.5} & \ctwo{261} & \cthree{1146.924} & \cthree{32.2 / 48.2 / 53.6} &	\cthree{4641}\\
%=======================================================================================================================================
\midrule
\multicolumn{11}{c}{Study case (s\&p noise) with average measurement error of \cone{108.21m} / \ctwo{121.78m} / \cthree{108.66m}}\\
\midrule
Baseline & 0 & \cone{65.301} & \cone{40.1 / 73.7 / 84.8} & \cone{0} & \ctwo{102.619} & \ctwo{35.2 / 60.3 / 70.7} & \ctwo{0} & \cthree{84.655} & \cthree{27.8 / 57.2 /73.0} & \cthree{0}\\
Ours     & 0 & \cone{2.066} & \cone{\textbf{64.8} / \textbf{92.1} / \textbf{97.6}} & \cone{0} & \ctwo{\textbf{7.707}} & \ctwo{76.3 / \textbf{93.3} / \textbf{97.0}} & \ctwo{0} & \cthree{\textbf{2.903}} & \cthree{\textbf{62.1} / \textbf{89.1} / \textbf{96.3}} & \cthree{0}\\ \midrule
Baseline & 1.0\% & \cone{\bf{0.948}} & \cone{43.6 / 79.5 / 91.4} & \cone{5.7} & \ctwo{3551.868} & \ctwo{24.5 / 36.6 / 40.1} & \ctwo{6437} & \cthree{724.908} & \cthree{14.5 /29.0 /37.2} & \cthree{6139}\\
Ours     & 1.0\% & \cone{505.969} & \cone{42.8 /	61.7 / 65.7} & \cone{32.6} & \ctwo{14.061} & \ctwo{\textbf{74.6} / 91.0 / 94.9} & \ctwo{237} & \cthree{119.592} & \cthree{44.5 / 66.4 / 72.6} &	\cthree{2716}\\ \midrule
Baseline & 2.5\% & \cone{436.084} & \cone{30.6 / 52.9 / 60.9} & \cone{38.8} & \ctwo{3552.177} & \ctwo{24.4 / 36.4 / 40.1} & \ctwo{6465} & \cthree{1388.735} & \cthree{1.1 / 2.0 / 2.9}	& \cthree{10442}\\
Ours     & 2.5\% & \cone{358.922} & \cone{40.5 / 57.4 / 61.1} & \cone{36.8} & \ctwo{13.76} & \ctwo{75.2 / 91.5 / 95.6} & \ctwo{254} & \cthree{920.801} & \cthree{29.8 / 44.1 / 50.0} &	\cthree{5061}\\

\bottomrule
\end{tabular}
%}
\end{center}
\end{table*}
 \setlength{\tabcolsep}{1.4pt}







% car coordinate
% % \setlength{\tabcolsep}{4pt}
% \begin{table*}[h]
% %\begin{table}[h]
% \centering
% \begin{center}
% \caption{Evaluation result of Unscented Kalman Filter}
% \label{table:eval_UKF}
% %\resizebox{\textwidth}{!}{
% \begin{tabular}{cccccccccc}
% \toprule
% Condition & \multicolumn{3}{c}{$Q^\text{sunny}$} & \multicolumn{3}{c}{$Q^\text{night}$} & \multicolumn{3}{c}{$Q^\text{snowy}$} \\
% \midrule
% Metric & $d_\text{err}$(m) & Cov-credibility(\%) & $n_r$ & $d_\text{err}$(m) & Cov-credibility(\%) & $n_r$ & $d_\text{err}$(m) & Cov-credibility(\%) & $n_r$\\
% \midrule
% Baseline & 0.765 & 46.0 / 81.2 / 92.2 & N/A & 8.254 & 38.3 / 67.0 / 78.9 & N/A & 1.302 & 30.5 / 61.7 / 79.6 & N/A\\
% Ours & 0.571 & 60.9 / 90.7 / 97.1 & N/A & 3.028 & 75.1 / 94.2 / 98.5 & N/A& 0.812 & 54.1 / 85.5 / 95.5 & N/A\\

% \bottomrule
% \end{tabular}
% %}
% \end{center}
% \end{table*}

==> tables/eval_measurement.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}
\begin{center}
\caption{Evaluation result on measurement}
\label{table:eval_measurement}
\begin{tabular}{ccc}
    \toprule
    Query Data & Uncertainty Error & Loc Error (m) \\ 
    \midrule
    $Q^\text{sunny}$  & 0.060 & 0.871  \\
    $Q^\text{night}$ & 0.109 & 8.680 \\
    $Q^\text{snowy}$ & 0.026 & 1.424 \\
\bottomrule 
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{1.4pt}

==> tables/eval_unseen.tex <==
%  \setlength{\tabcolsep}{2.5pt}
% \begin{table}[!bt]
% \centering
% \caption{Evaluation results of expected calibration error for unseen locations (data A) under sunny condition. Lower is better.}
% \label{table:eval_unseen_ECE_sunny}
% \begin{tabular}{lcccc}
% \toprule

% Sensor error model & Downtown & Highway& Rural area & Campus \\
% \midrule 
% Using data B & 5.07\% & 8.62\% & 2.45\% & 8.37\%   \\
% Using data A and B & 7.35\% & 9.35\% & 1.08\% & 9.06\%  \\

% \bottomrule
% \end{tabular}
% \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 
%  \setlength{\tabcolsep}{2.5pt}
% \begin{table}[!bt]
% \centering
% \caption{Evaluation results of expected calibration error for unseen locations (data A) under night condition. Lower is better.}
% \label{table:eval_unseen_ECE_night}
% \begin{tabular}{lcccc}
% \toprule

% Sensor error model & Downtown & Highway& Rural area & Campus \\
% \midrule 
%  Using data B & 1.13\% & 14.38\% & 6.63\% & 4.80\%   \\
% Using data A and B & 1.80\% & 15.01\% & 7.92\% & 7.34\%   \\

% \bottomrule
% \end{tabular}
% \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 \setlength{\tabcolsep}{2.5pt}
\begin{table}[!bt]
\centering
\caption{Evaluation results of expected calibration error for unseen locations (set A). Lower is better.}
\label{table:eval_unseen_ECE}
\begin{tabular}{clcccc}
\toprule

Condition & Sensor error model & Downtown & Highway& Rural area & Campus \\
\bottomrule
\multirow{2}{*}{Sunny} & Using set B & 5.07\% & 8.62\% & 2.45\% & 8.37\%   \\
& Using set A and B & 7.35\% & 9.35\% & 1.08\% & 9.06\%  \\
\midrule
\multirow{2}{*}{Night} & Using set B & 1.13\% & 14.38\% & 6.63\% & 4.80\%   \\
& Using set A and B & 1.80\% & 15.01\% & 7.92\% & 7.34\%   \\
\midrule
\multirow{2}{*}{Snowy} & Using set B & 5.10\% & 4.56\% & 1.28\% & 7.55\%   \\
 & Using set A and B & 3.05\% & 3.70\% & 2.09\% & 7.89\%    \\

\bottomrule
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \setlength{\tabcolsep}{2.5pt}
\begin{table}[!bt]
\centering
\caption{Evaluation results of Sigma Point Filter localization for unseen location (set A).}
\label{table:eval_UKF_unseen}
\begin{tabular}{cclcc}
\toprule
Condition & Area & Method & $d_\text{err}$(m) $\downarrow$ & Cov-credibility(\%) \\ 
\bottomrule

\multirow{8}{*}{Sunny} & \multirow{2}{*}{Downtown} & Using set B  & 0.472 &
54.4 / 89.4 / 97.4
  \\
& & Using set A and B & 0.466 & 
60.9 / 92.5 / 98.4
  \\
\cmidrule{2-5}

 & \multirow{2}{*}{Highway} & Using set B  & 0.579 &
71.9 / 95.0 / 99.0
  \\
& & Using set A and B & 0.569 &
73.8 / 95.6 / 99.1
  \\
\cmidrule{2-5}

 & \multirow{2}{*}{Rural area} & Using set B  & 0.736 &
46.0 / 80.6 / 95.1
  \\
& & Using set A and B & 0.732 &
49.9 / 84.6 / 95.5
  \\
\cmidrule{2-5}

 & \multirow{2}{*}{Campus} & Using set B  & 0.556 &
63.7 / 94.9 / 98.6 
  \\
& & Using set A and B & 0.551 & 
67.0 / 95.7 / 99.4
  \\
\bottomrule

%%%%%%
\multirow{8}{*}{Night} & \multirow{2}{*}{Downtown} & Using set B  & 0.620 & 46.1 / 81.9 / 95.6 
  \\
& & Using set A and B & 0.614 &
51.1 / 85.1 / 97.2

  \\
\cmidrule{2-5}

& \multirow{2}{*}{Highway} & Using set B  & 1.957 & 90.3 / 98.7 / 99.8
  \\
& & Using set A and B & 2.580 & 
89.1 / 99.4 / 99.9
  \\
\cmidrule{2-5}

& \multirow{2}{*}{Rural area} & Using set B  & 5.642 & 70.8 / 92.9 / 98.5
  \\
&  & Using set A and B & 5.543 & 
81.0 / 96.4 / 99.2

  \\
\cmidrule{2-5}

& \multirow{2}{*}{Campus} & Using set B  & 0.936 & 47.9 / 91.5 / 99.4

  \\
& & Using set A and B & 0.937 &
60.2 / 98.2 / 100.0 \\

\bottomrule
%%%%%%

\multirow{8}{*}{Snowy} & \multirow{2}{*}{Downtown} & Using set B  & 0.793 & 38.4 / 73.7 / 91.5
  \\
& & Using set A and B & 0.787 &
42.4 / 78.5 / 93.1
  \\
\cmidrule{2-5}

 & \multirow{2}{*}{Highway} & Using set B  & 1.209 & 41.8 / 76.1 / 92.0
  \\
& & Using set A and B &1.183 &
44.3 / 78.3 / 93.4

  \\
\cmidrule{2-5}

 & \multirow{2}{*}{Rural area} & Using set B  & 0.886&49.0 / 84.5 / 94.8

  \\
& & Using set A and B & 0.882&
52.6 / 85.2 / 95.2


  \\
\cmidrule{2-5}

 & \multirow{2}{*}{Campus} & Using set B  & 0.670 & 57.9 / 90.5 / 98.0


  \\
&  & Using set A and B & 0.664 & 
60.0 / 91.7 / 98.2


  \\
\bottomrule
\end{tabular}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \setlength{\tabcolsep}{2.5pt}
% \begin{table}[!bt]
% \centering
% \caption{Evaluation results of Sigma Point Filter localization for unseen location (data A) under sunny condition.}
% \label{table:eval_UKF_unseen_sunny}
% \begin{tabular}{clcc}
% \toprule
%  Area & Method & $d_\text{err}$(m) $\downarrow$ & Cov-credibility(\%) \\ 
% \midrule 

% \multirow{2}{*}{Downtown} & Using data B  & 0.472 &
% 54.4 / 89.4 / 97.4
%   \\
%  & Using data A and B & 0.466 & 
% 60.9 / 92.5 / 98.4
%   \\
% \midrule

% \multirow{2}{*}{Highway} & Using data B  & 0.579 &
% 71.9 / 95.0 / 99.0
%   \\
%  & Using data A and B & 0.569 &
% 73.8 / 95.6 / 99.1
%   \\
% \midrule

% \multirow{2}{*}{Rural area} & Using data B  & 0.736 &
% 46.0 / 80.6 / 95.1
%   \\
%  & Using data A and B & 0.732 &
% 49.9 / 84.6 / 95.5
%   \\
% \midrule

% \multirow{2}{*}{Campus} & Using data B  & 0.556 &
% 63.7 / 94.9 / 98.6 
%   \\
%  & Using data A and B & 0.551 & 
% 67.0 / 95.7 / 99.4
%   \\
% \bottomrule
% \end{tabular}
% \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \setlength{\tabcolsep}{2.5pt}
% \begin{table}[!bt]
% \centering
% \caption{Evaluation results of Sigma Point Filter localization for unseen location (data A) under night condition.}
% \label{table:eval_UKF_unseen_night}
% \begin{tabular}{clcc}
% \toprule
%  Area & Method & $d_\text{err}$(m) $\downarrow$ & Cov-credibility(\%) \\ 
% \midrule 

% \multirow{2}{*}{Downtown} & Using data B  & 0.620 & 46.1 / 81.9 / 95.6 
%   \\
%  & Using data A and B & 0.614 &
% 51.1 / 85.1 / 97.2

%   \\
% \midrule

% \multirow{2}{*}{Highway} & Using data B  & 1.957 & 90.3 / 98.7 / 99.8
%   \\
%  & Using data A and B & 2.580 & 
% 89.1 / 99.4 / 99.9
%   \\
% \midrule

% \multirow{2}{*}{Rural area} & Using data B  & 5.642 & 70.8 / 92.9 / 98.5
%   \\
%  & Using data A and B & 5.543 & 
% 81.0 / 96.4 / 99.2

%   \\
% \midrule

% \multirow{2}{*}{Campus} & Using data B  & 0.936 & 47.9 / 91.5 / 99.4

%   \\
%  & Using data A and B & 0.937 &
% 60.2 / 98.2 / 100.0

%   \\
% \bottomrule
% \end{tabular}
% \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \setlength{\tabcolsep}{2.5pt}
% \begin{table}[!bt]
% \centering
% \caption{Evaluation results of Sigma Point Filter localization for unseen location (data A) under snowy condition.}
% \label{table:eval_UKF_unseen_snowy}
% \begin{tabular}{clcc}
% \toprule
%  Area & Method & $d_\text{err}$(m) $\downarrow$ & Cov-credibility(\%) \\ 
% \midrule 

% \multirow{2}{*}{Downtown} & Using data B  & 0.793 & 38.4 / 73.7 / 91.5
%   \\
%  & Using data A and B & 0.787 &
% 42.4 / 78.5 / 93.1
%   \\
% \midrule

% \multirow{2}{*}{Highway} & Using data B  & 1.209 & 41.8 / 76.1 / 92.0
%   \\
%  & Using data A and B &1.183 &
% 44.3 / 78.3 / 93.4

%   \\
% \midrule

% \multirow{2}{*}{Rural area} & Using data B  & 0.886&49.0 / 84.5 / 94.8

%   \\
%  & Using data A and B & 0.882&
% 52.6 / 85.2 / 95.2


%   \\
% \midrule

% \multirow{2}{*}{Campus} & Using data B  & 0.670 & 57.9 / 90.5 / 98.0


%   \\
%  & Using data A and B & 0.664 & 
% 60.0 / 91.7 / 98.2


%   \\
% \bottomrule
% \end{tabular}
% \end{table}
